Higher Order Maximum Persistency and Comparison Theorems

We address combinatorial problems that can be formulated as minimization of a partially separable function of discrete variables (energy minimization in graphical models, weighted constraint satisfaction, pseudo-Boolean optimization, 0-1 polynomial programming). For polyhedral relaxations of such problems it is generally not true that variables integer in the relaxed solution will retain the same values in the optimal discrete solution. Those which do are called persistent. Such persistent variables define a part of a globally optimal solution. Once identified, they can be excluded from the problem, reducing its size. To any polyhedral relaxation we associate a sufficient condition proving persistency of a subset of variables. We set up a specially constructed linear program which determines the set of persistent variables maximal with respect to the relaxation. The condition improves as the relaxation is tightened and possesses all its invariances. The proposed framework explains a variety of existing methods originating from different areas of research and based on different principles. A theoretical comparison is established that relates these methods to the standard linear relaxation and proves that the proposed technique identifies same or larger set of persistent variables.

==> acknowlegement.tex <==
\section*{Acknowlegement}


==> future.tex <==
\subsection{Open Questions}

\paragraph{Improving = Relaxed-Improving for Tractable Languages?}

Ok, actually the first question here is this. If the relaxation is tight, then the mapping that sends everything to an optimal integer solution $x^*$ is relaxed improving or not? If it was not, then exists $\mu$ such that $\<f, \mu\> < \<f,\delta(x^*)\>$, a contradiction. So it must be relaxed-improving. But what about other improving maps, \eg $x\mapsto x \vee x^*$ for submodular functions. Are they relaxed-improving?

\par
%A new proof chain to close the question on all these submodular bisubmodular scuffling.
In the comparison theorem for bisubmodular functions, it seems that the key property is that it belongs to the tractable class, solved exactly by BLP. To generalize to the full tractable class we lack only that an improving mapping can be proven to be relaxed-improving. It would be actually a strong result in itself, it can be formally stated as follows.
\begin{theorem} Let $f$ be from a tractable language and $p\colon \X\to \X$ an improving component-wise mapping. Then $p$ is BLP-improving for $f$.
\end{theorem}
\begin{proof}
Assume for contradiction that $p\notin\WI$. On one side we have
$$
\min_{\mu\in\Lambda} \<f,\mu \>
$$
integral and
$$
(\forall \mu\in\M)\ \ \<f,P\mu\> \leq \<f,\mu\>
$$
On the other side
$$
\min_{\mu\in\Lambda} \<(I-P\T)f,\mu \> < 0. 
$$
It means $\mu$ is not integral and $\<f,\mu \> < \< f, P \mu \>$.
%there exists $\mu\in\Lambda$ such that $\<f, [p] \mu \> > \<f,\mu\>$. But $\mu' = [p] \mu \in\Lambda$ and therefore $\<f, \mu' \> > \<f,\mu\>$.
By characterization theorems
$$
\inf_{A \mu =0,\ \mu\geq 0} \<(I-P\T)f,\mu \> = -\infty. 
$$
$$
\inf_{A (I-P) \mu = 0,\ \mu\geq 0} \<f,(I-P) \mu \> = -\infty. 
$$
$$
(\not\exists \varphi) \ \ (I-P\T) (f - A\T \varphi) \geq 0.
$$
\end{proof}
\begin{proof}
This is an open question. Some ideas follow.
%If $f$ is in tractable class, 
%Assume for contradiction that $\exists \mu\in\Lambda$ such that $<(I-P\T)f, \mu> < 0$
We inspect the verification problem
$$
\min_{\mu\in\Lambda} \<(I-P\T)f,\mu \>
$$
and try to see if it is from a tractable language too. If the optimal solution is integer, the value is equal to the minimization over $\M$ for which we know the optimum is zero.
\par
So unary terms $(I-P\T)f_s$ do not matter. What about higher order terms, how their change affects tractability?
Through the new reduction theorem? What it does is grouping of labels and submodularity enforcement. Need to show that submodularity enforecement does not break tractability. Does not break skew-submodularity or what is the characterization.
\end{proof}
The generalized comparison theorem then will have then the following form:
\begin{theorem}
Let $\pi \colon \X \to \X'$ be component-wise injection so that $f_e(x_e) = f'_e(\pi_e(x_e))$ holds. Let $f'$ be from a tractable language. Let $p'$ be a component-wise improving map for $f'$. Let $p$ be such that $\pi \circ p = p' \circ \pi$. Then $p$ is BLP-improving for $f$.
\end{theorem}
\par
\paragraph{Is \maxwi for higher order pseudo-Boolean in the P class?}
Problem \maxwi for higher order pseudo-Boolean case is not resolved. Indeed, we showed how to solve it for $\P^{1,y}$ and \maxsi problem for $\P^{1}$. Polynomiality of \maxwi for $\P^1$ is an open question. For higher order there is no such direct relation between relaxed solution with minimum / maximum number of integer components and \maxsi / \maxwi. Indeed \maxsi chooses a subset of variables from the minimum integer part. What about \maxwi ? Because applying the persistency results in a feasible optimal relaxed solution, \maxwi will fix a subset of the maximum integer part. We can prove a result similar to Picard and Queranne, that two relaxed improving maps $p$, $q$, when composed, produce a map who's persistency is the union of persistencies of $p$ and $q$. Then by fixing one variable at a time we get a polynomial algorithm if only we can verify weak persistency with a fixation exists. %Is there an efficient algorithm? 
I proved the problem is NP-hard. But composing $p$ and $q$ is interesting. All maximal solutions are global?

==> revision.tex <==

\twocolumn[
  \begin{@twocolumnfalse}
    %\maketitle
\begin{center}
\Large Response to Reviews
\vskip10pt
\end{center}    
  \end{@twocolumnfalse}
]

I thank the reviewers for their very constructive response, which helped significantly to improve technical correctness and clarity of the paper, in particular the construction of the persistency linear program.
\vskip10pt

\paragraph{Reviewer1:}
The experimental results are very impressive. The only thing I am missing is the running times for all the algorithms, and a short discussion of what the practical limits are and how they can be overcome.
\begin{itemize}
\blue
\item[\checkmark] Added plot of running times in \Figure{f:exp-rand-h2} and discussion of efficient methods in \Section{sec:discussion}.
\end{itemize}

{- What happens if you run your algorithm iteratively - do you get more persistencies then?}
\begin{itemize}
\blue
\item[\checkmark]
A discussion to this interesting question is added in~\Section{sec:discussion}. A relevant example for BLP relaxation in \Figure{fig:BLP} explains why generalized roof duality, which works iteratively, may become better than the maximum BLP-improving map.
\end{itemize}
{
- Explanations of illustrations should be provided. The figs 1-4 are good, but it takes some time to digest what they are depicting. Avoid having letters like t', t, s which are not needed or referenced.
}
\begin{itemize}
\blue
\item[\checkmark] Figures have been cleaned up and explanation improved, new \Figure{fig:energy} explains the graphical notation.
\end{itemize}
\par
- Line 297-304. This is a very important conclusion and should be highlighted (statement?) and elaborated upon.
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

- \Lemma{L:coni-Lambda}. Provide a definition of "conic hull" to make the paper more self-contained. Regarding proof, there are not two "directions", you prove that one is a subset of the other and vice versa.
\begin{itemize}
\blue
\item[\checkmark] The definition, the lemma and its proof were clarified.
\end{itemize}

- \Lemma{necessary-LI}. Previously it is said that [p] will only mean "node-wise", so it is a bit confusing why "component-wise" is introduced here.
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

- \Statement{S:WI-dual}. You should explain in the statement what the A in the definition of $f^\varphi$ stands for or give reference. For convenience, it would be good to repeat the definition of $f^\varphi$ as well. Proof: Condition (20) on its own is not equivalent to (18).
\begin{itemize}
\blue
\item[\checkmark] corrected
\end{itemize}

- Why is \ref{S:WI-dual} statement and \ref{S:SI-dual} theorem?
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

- Line 397-405. The explanations of maps can be made clearer and more strict. Suggestions: Elaborate on $P^{1,y}$. "$y_s$ is free" - what does that mean? Why the superscript 1 and 2 for $P$?
\begin{itemize}
\blue
\item[\checkmark] Clarified and better motivated, see updated~\Section{sec:maximum persistency}. Superscripts 1,2 are just for enumeration, no mathematical meaning.
\end{itemize}

- [20] has appeared in a journal (DAM). [21] and [70] are duplicates.
\begin{itemize}
\blue
\item[\checkmark] for all CoRR
\end{itemize}

- Rename Section 7 to Appendix.
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

- Typos:

L. 104, "extension" -> "extensions"
L. 196, wrong font on "c"
L. 253, 2nd col, "in in"
L. 589, 2cd col, "pursuit" is a noun.
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}


\paragraph{Reviewer2:}
165R: The NP-hardness part was proved in
J. Thapper, S. Zivny. The complexity of finite-valued CSPs. STOC 2013.
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

220L: $\delta(L)$ $\Rightarrow$ $\delta(X)$
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

282L: "no power of p is guaranteed to be idempotent". Is it true?
Let $X'\subseteq X$ be the set of all elements that cycle, and
for $x\in X'$ let $n(x)$ be the length of the cycle. Now take n to be the gcd
of $n(x)$ for $x\in X'$. Wouldn't $p^n$ be idempotent?
\begin{itemize}
\blue
\item[\checkmark] Thanks for the tip, the explanation in \Section{subsec:improving-map} was improved.
\end{itemize}

250R: check English. ( "there will retaining ..." )
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

253R: "in in"
\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

306L: I can see why $W_f$ is an interesection of finitely many half-spaces:
it suffices to consider inequalities for mu's that are corners of $\Lambda$.
Is it obvious that $S_f$ is an intersection of *finitely many* open half-spaces?
Before talking about polytopes, you may want to say that mapping P is
homogeneous, and will be represented by a matrix of size $|I|\times |I|$
(and so $P$ belongs to $R^d$).
\begin{itemize}
\blue
\item[\checkmark] The text in question was not essential and now is removed. \Theorem{S:SI-dual} encloses the finate set of discrete maps of our interest $\{[p] \in\SI \mid p\colon \X\to\X \}$ in a closed polytope as discussed now after the theorem.
\end{itemize}

I had a hard time going through section 2.5.

406L: "numbers $P_{C,x_C,x_{C'}}$ are expressed as ..."
As far as see, these numbers were never defined before.
Eq. (34) could serve as a definition, but it is given
later. Please rephrase, e.g. "let us defined numbers ... as ..."
\begin{itemize}
\blue
\item[\checkmark] Now defined in~\eqref{pixel-ext-comp}.
\end{itemize}

Eq. (34): Does $x'_D$ means the restriction of $x'_C$ to $D$?
I believe this convention was never described, you may
want to say it here (if that's the first time it is used).
\begin{itemize}
\blue
\item[\checkmark] Now defined in~\Section{sec:energy}.
\end{itemize}

Eq. (36) and the preceding paragraph were extremely hard
to follow. One problem for me was that in the beginning
A, B are defined as fixed sets, but in eq. (36) they
are quantified over, without any explanation.
It took me a long time to come with the following
intepretation: you claim that for each $A,B\in C$ and $x'_D$
there exists $x_D$ such that eq. (36) for this $A,B$ is equivalent to
to the constraint $P_{C,x_C,x'_{C}} \ge 0$, and therefore
the set of inequalities (36) for all $A,B\in C$
is equivalent to the set of inequalities $P_{C,x_C,x'_{C}} \ge 0$
for all $x_C$. Is it true? What if there are two possible labels
and $x'_s \ne y_s$? Then sets $A,B$ would not be independent.
\begin{itemize}
\blue
\item[\checkmark] This is a correct observation. The claim appears to hold despite $A,B$ are not independent as proven now in \Theorem{T:SA-equiv}. At the same time construction of L1 after the revision builds on the relaxation of Sherali-Adams directly and not on this claim.
\end{itemize}


438L: "Let us detail $P_{C,x_C,x_{C'}}$". It would be clearer to me to say
"let us detail the constraint $P_{C,x_C,x_{C'}} \ge 0$" (if that's what you mean).

\begin{itemize}
\blue
\item[\checkmark] Now defined in~\Section{sec:energy}.
\end{itemize}

You should not assume that the reader is familiar with the Sherali-Adams relaxation.
E.g. what exactly it relaxes? A more natural way to introduce this could be as follows:
after (33) and (34) add "with the constraints $\zeta_{D,x_D}=\prod_{s\in D}\zeta_{s,x_s}$.
We use a Sherali-Adams relaxation of these non-linear constraints given by (36)".
(Is it what you do?)
Then you can say that these constraints imply eq. (35a).
\begin{itemize}
\blue
\item[\checkmark] It turns out the initial construction was essentially introducing a relaxation equivalent to the one by Sherali and Adams and referencing their integrality theorem. By the suggestion of the reviewer, the revision now builds on the relaxation of Sherali-Adams directly. Hopefully it is more clear now. A short summary of key points of relaxation of Sherali-Adams is now introduced in \Section{sec:SA-relaxation}. Clarifying what exactly it relaxes and its properties allowed to significantly shorten some of the subsequent proofs.
\end{itemize}

444L: (32) and (33) use products of $\zeta_s$ variables while (36)
uses $\zeta_D$ variables. Of course, for integer values they coincide,
but since you use a relaxation, you may want to be more consistent.

\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

Statement 2.10: Eq. (53) is defined several pages later. Is it a wrong reference?

\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

458R: "thus making ... solvable". This argument is incomplete: does \Theorem{T LP1 tight}
still holds after adding additional constraints on $\zeta$?
\begin{itemize}
\blue
\item[\checkmark] A justification is added in~\Section{sec:two-phase} and the proof of \Theorem{T LP1 tight} is moved to the main part of the paper to make this argument clear.
\end{itemize}

Eq. (44): To specify relation "subsetdot", you also need to say for which sets $C$
you add the constraint.

\begin{itemize}
\blue
\item[\checkmark]
\end{itemize}

For my taste, the introduction of \Section{sec:comparison} has too much text, and so overall it sounds a bit vague.
An (optional) suggestion is to list concrete questions that you study, e.g. something along the following lines:
- compare the number of persistent nodes given by your Algorithm 2 and by algorithm X
\begin{itemize}
\blue
\item[\checkmark] \Section{sec:comparison} was revisited. Vague discussion removed and summary of concrete results is given in Table~\ref{table:comparisons}.
\end{itemize}
- study which transformations of the energy function and/or relaxation preserve/weaken improving maps (and define what
it means; for example, it was not very clear to me what do you mean by "weaken" in \autoref{T:quad-weaken1}).
- ?
\begin{itemize}
\blue
\item[\checkmark] The theoretical comparison to quadratization techniques has been revisited(~\Section{sec:quadratization}~\Section{sec:hocr-proof}). Unclear term "weaken" is replaced with \Definition{def:maps-inclusion}. Theorems \ref{T:quad-preserve},~\ref{T:quad-weaken1},~\ref{T:quad-weaken2} are restated and their proofs detailed.
\end{itemize}


Experiments: can you say something about running times? Which LP solver did you use?
\begin{itemize}
\blue
\item[\checkmark] Added times plots in \Figure{f:exp-rand-h2}, see also its description in \Section{sec:evaluation}.
\end{itemize}
